A Weight-scaling Algorithm for $f$-factors of Multigraphs

We discuss combinatorial algorithms for finding a maximum weight $f$-factor on an arbitrary multigraph, for given integral weights of magnitude at most $W$. For simple bipartite graphs the best-known time bound is $O(n^{2/3}\, m\, \log nW)$ (\cite{GT89}; $n$ and $m$ are respectively the number of vertices and edges). A recent algorithm of Duan and He et al. \cite{DHZ} for $f$-factors of simple graphs comes within logarithmic factors of this bound, $\widetilde{O} (n^{2/3}\, m\, \log W)$. The best-known bound for bipartite multigraphs is $O(\sqrt {\Phi}\, m\, \log \Phi W)$ ($\Phi\le m$ is the size of the $f$-factor, $\Phi=\sum_{v\in V}f(v)/2$). This bound is more general than the restriction to simple graphs, and is even superior on "small" simple graphs, i.e., $\Phi=o(n^{4/3})$. We present an algorithm that comes within a $\sqrt {\log \Phi}$ factor of this bound, i.e., $O(\sqrt {\Phi \log \Phi}\,m \,\log \Phi W)$. The algorithm is a direct generalization of the algorithm of Gabow and Tarjan \cite{GT} for the special case of ordinary matching ($f\equiv 1$). We present our algorithm first for ordinary matching, as the analysis is a simplified version of \cite{GT}. Furthermore the algorithm and analysis both get incorporated without modification into the multigraph algorithm. To extend these ideas to $f$-factors, the first step is "expanding" edges (i.e., replacing an edge by a length 3 alternating path). \cite{DHZ} uses a one-time expansion of the entire graph. Our algorithm keeps the graph small by only expanding selected edges, and "compressing" them back to their original source when no longer needed. Several other ideas are needed, including a relaxation of the notion of "blossom" to e-blossom ("expanded blossom").

==> Falg.tex <==
\subsection*{Overall Algorithm: The Scaling Loop}
Our overall algorithm is a scaling loop. Here we follow the 
description in \cite{DPS}.
Take $W$ so that the given weight function,
denoted $\widehat w$, takes on integral values in $[0,W]$.
(Negative weights are easily eliminated since every perfect matching of
$G-v$ has cardinality $\f{n/2}$.)
Define a  derived weight function by
$\overline w =     % \frac{n+3}{2} \hat w$.
(n+1)\widehat w$.
The algorithm operates in 
%$s=\f{\log_2 \frac{n+3}{2} W}$
$s=\f{\log (n+1) W}$ scales.
For $i=1,\ldots, s$, the $i$th scale
finds a near-optimum structured matching
for the  weight function 
\[w(e)=2\times(\text{the leading $i$ bits of }\overline w(e)).\]

To justify this outline note that any value $\overline w(e)$ 
\iffalse
The final matching is optimum for the given weight function $\hat w$.
= \frac{n+3}{2} \hat w(e)\le
\frac{n+3}{2} W$ is an integer of $\le \log 
\frac{n+1}{2} W$ is an integer of 
$\le \f{\log_2 \frac{n+1}{2} W}+1 =\f{\log_2 \frac{n+1}{2} W}+1 
\fi
is at most $(n+1) W$, 
so it is an integer of
$\le \f{\log (n+1)W}+1$   % =\f{\log_2 \frac{n+1}{2} W}+1 
bits. The last bit is 0 ($n+1$ is even).
So the $s$th scale uses the weight function  $(n+1) \widehat w$,
and it gives the desired near-optimum structured matching.






\iffalse
In general for
any mpr $R\con V$, \algcall DismantlePath(R) works as follows:

\bigskip

for each maximal mpr $Q\pcon R$, in bottom up order,  do \algcall DismantlePath(Q)

%execute Phases 1--3 

if $R=V$ then

{\hi $z(V)\gets n^2 W$

  $/*$ $V$ now consists of one (odd) shell,
  with $\Omega^-=\emptyset$ and an arbitrary number of free vertices $*/$

  reexecute Phases 1--3

$/*$ no shell dissolves, so Phase 3 makes $V$ a blossom $*/$

}
\bigskip

The assignment to $z(V)$ is just for uniformity. It ensures every
vertex will become outer before $V$ dissolves, i.e., the algorithm
halts with $V$ a blossom.
\fi

\iffalse
%%%%%%%%%%%%%%% DISCARDS%%%%%%%%%%%%%%%%%%
{\parindent=0pt

{\bf Algorithm}

\bigskip

\algcall DismantlePath(R) has 3 steps and uses \algname ShellSearch1. and 
\algname ShellSearch2.:

1. While $|F|>\sqrt {n(R)}$:

{\hi

    as before sort the undissolved shells on $\#$ free vertices
 
    and execute \algcall ShellSearch1(S_i) in decreasing size order
}

\bigskip

2. While $|F|>1$:

{\hi

    let $C,D$ be the outermost shell with free vertices

    execute \algcall ShellSearch2(C,D) (to augment the matching)

}

\bigskip

3. $|F|=1$: proceed as before

\bigskip

\algcall ShellSearch1(C,D):

if $(C,D)$ is a big shell then

{\hi
  do \algname SearchOne. (Criterion 2) on (C,D)
}

else ($(C,D)$ is a small shell)

{\hi
  do \algname BucketSearch. (Criterion 3) on $G\shell(C,D)$

{\hi
  stop when either

{\hi
     an augmenting path is found -- augment the matching

     or

     C or D dissolves
}}}

\bigskip

\algcall ShellSearch2(C,D):

Do \algname BucketSearch. (Criterion 3) to find  augmenting path

{\hi
   (enlarge active region to C*,D* as before) 
}

\bigskip

{\bf Perfection Step}

Assume the graph is critical, so \algname DismantlePath. does everything.

}

\fi


==> newed.tex <==
\section{Edmonds' algorithm and its implementation}
\label{ReviewSec} 

\def\fm.{$min\_edge$}
\def\fms.{$min\_edges$}

This section summarizes Edmonds' algorithm  and 
known results on its implementation.
Sections \ref{BlossomSec}--\ref{EdAlgSec}
sketch the high level algorithm.
They include all 
the details needed for our implementation but
do not give a complete development.
For the latter see, e.g., 
\cite{E, G73, L, PS}.
%Also Appendix \ref{EdAppendix}
%gives complete pseudcode for the  search algorithm.
Section \ref{BMergingSec} 
reviews the portions of the algorithm
for which efficient implementations are known, and 
the outstanding problem of efficient ``blossom merging''.

\begin{figure}[th]
\centering
\input{1Fig.pstex_t}
%save the fig at magnification 60%
%{\epsfig{figure=1Fig.eps, width=2.5in}}
%{\epsfig{figure=1Fig.pstex_t, width=4.5in}}
%{\epsfig{figure=1Fig.pstex, width=4.5in}}
 \caption{Blossoms in a search of Edmonds' algorithm.
Blossom $B$ is formed from subblossoms $B_0,\ldots,B_6$.
Heavy edges are matched.}
 \label{1Fig}
 \end{figure}

\subsection{Blossoms}
\label{BlossomSec} 
Throughout this section the notation $P(x,y)$ denotes an $xy$-path.
This includes the possibility that $x=y$, i.e., $P(x,x)=(x)$.

Edmonds' algorithm is based on the notion of blossom.
We start with a data-structure-oriented definition,
illustrated in  Fig.~\ref{1Fig}.
Begin by considering two even-length alternating paths $P(x_i,y)$,
 $i=0,1$,
with $x_0\ne x_1$ and $y$ the only common vertex. 
Each path begins  with the matched edge at $x_i$, unless $x_i=y$. 
These paths plus an edge $x_0x_1$ form a simple example of a blossom.
Edmonds' algorithm contracts blossoms. This leads to the general, recursive
 definition:

\begin{definition}
\label{BlossomDefn}
Let $G$ be a graph with a distinguished matching.
A {\em blossom} is a subgraph defined by rules (a) and (b):
 
(a) Any single vertex $b$ is a blossom. 

(b) Let $\oG$ be a graph formed from $G$ by contracting zero or more
vertex-disjoint blossoms.
Let $X_0,X_1,Y$ be $\oG$-vertices, $X_0\ne X_1$.
For
$i=0,1$ let
 $P(X_i,Y)$ be an even-length alternating path that starts with a 
matched
edge or has $X_i=Y$, 
with $Y$ the only common 
$\oG$-vertex.
These paths plus an edge $X_0X_1$ form a blossom. 
\end{definition}

In Fig.~\ref{1Fig} blossom $B$ is formed from
paths $P(B_4,B_0)$, $P(B_6,B_0)$ and edge $\gamma$.
We use the term ``vertex'' to refer to a vertex of the given graph $G$.
For a blossom $B$, $V(B)$ is
the set of vertices of $G$ contained in
any blossom in either path $P(X_i,Y)$;
we sometimes refer to them as {\em the vertices of $B$}.
The maximal blossoms in the paths $P(X_i,Y)$
are {\em the subblossoms of $B$}.



We use some properties of blossoms 
that are easily established by induction.
Any blossom has a {\em base vertex}: In 
Definition \ref{BlossomDefn}
a blossom of type (a) has base vertex $b$.
A blossom of type (b) has the same base vertex as $Y$.
We usually denote the base of $B$ as $\beta(B)$
(or $\beta$ if the blossom is clear). $\beta(B)$
is the unique vertex of $B$ that is not
matched to another vertex of $B$.
$\beta(B)$ is either free or matched to a vertex
not in $B$.
We call $B$ a {\em free blossom} or {\em matched blossom}
accordingly.

Consider a blossom $B$ with base vertex $\beta$.
Any vertex $x\in V(B)$ has an even-length alternating path
$P(x,\beta)$ that starts with the matched edge at $x$.
($P(\beta,\beta)$ has no edges.)
For example in Fig.\ref{1Fig} in blossom $B$, $P(a,\beta(B))$
starts with $P(a,\beta(B_1)) =(a_0,a_1,a_2,a_3,a_4)$
followed by edge $(\beta(B_1),\beta(B_2))$ and the reverse of 
$P(c,\beta(B_2))$,
and continuing along paths in $B_3,B_4,B_6,B_5,B_0$.

To define  $P(x,\beta)$
in general
consider the two paths
for $B$ in Definition \ref{BlossomDefn}.
Among the blossoms in these  paths
let $x$ belong to a blossom designated as $B_0$.
The edges of $B$ (i.e., the edges of $P(X_i,Y)$
plus $X_0X_1$) contain a unique even-length alternating path $A$
from $B_0$ to $Y$. Here $A$ is a path in $\o G$. 

First suppose
$B_0\ne Y$. $A$
starts with the matched edge at $B_0$.
$P(x,\beta)$ passes through the same blossoms as $A$.
To be precise let the $\o G$-vertices of
$A$ be $B_i, i=0,\ldots,k$, $B_k=Y$, with $k>0$ even.
Let $\beta_i$ be the base vertex of $B_i$.
So there are vertices $x_i\in V(B_i)$ such that 
the edges of $A$ are 
\[
%$\beta_0\beta_1$, $x_1x_2$,  $\beta_2\beta_3$, $x_3x_4$,\ldots, $x_{k-1}x_k$.  
\beta_0\beta_1,  x_1x_2 ,   \beta_2\beta_3 ,  x_3x_4 ,\ldots,  x_{k-1}x_k .  
\]
Here the $\beta_i\beta_{i+1}$ edges are matched 
and the $x_ix_{i+1}$ edges are unmatched.
Recursively define  $P(x,\beta)$ as the concatenation of $k+1$ subpaths 
\begin{equation}
\label{PvbEqn}
P(x,\beta)= P(x,\beta_0), P(\beta_1,x_1),P(x_2,\beta_2),P(\beta_3,x_3),\ldots,
P(x_k,\beta_k).
\end{equation}
%$x_i$ is the vertex of $B_i$ on the unmatched edge of $A$ incident to $B_i$.
For odd $i$, $P(\beta_i,x_i)$ is the reverse of path $P(x_i,\beta_i)$.

Now consider the base case
$B_0=Y$. If $Y$ is a vertex then $Y=x=\beta$
and $P(x,\beta)=(x)$. Otherwise $P(x,\beta)$ in blossom $B$ is identical
to $P(x,\beta)$ in $B_0$.%
\footnote{The $P(x,\beta)$ paths may intersect in nontrivial ways.
For instance in Fig.~\ref{1Fig}, $P(\beta(B_3),\beta(B))$ and $P(\beta(B_5),\beta(B))$
traverse edge $\gamma$ in opposite directions. 
So the paths have common subpaths, e.g., the subpath
of $P(\beta(B_5),\beta(B))$ joining $\gamma$ and edge $(\beta(B_3),\beta(B_4))$,
and disjoint subpaths, e.g., the subpath of $P(\beta(B_5),\beta(B))$
joining $\beta(B_3)$ and edge $\alpha$. This intersection pattern can continue
inside blossom $B_0$.
 So in general for two
vertices $x_0,x_1$ in a blossom $B$ with base $\beta$, the paths
$P(x_i,\beta)$ can have arbitrarily many subpaths that are alternately
common and disjoint.}

\iffalse
(This proof sketch does not
supply a precise definition of $P(x,b)$, but it
can be found in [GMG] and others.)
\fi

\iffalse
READ THIS

5/12/16:
i read it, seems no longer needed as more details than what's in this
have been included

We add one more detail to our sketch of Edmonds' algorithm.  Consider
a blossom $B$ with base vertex $b$ (in Figure 1 see vertex $w$ in
$B_1$).  Any vertex $x \in B$ is joined to the base $b$ by an
even-length alternating path of edges in $B$, which we denote as
$P(x,w)$.  (In Figure 1, $P(u,w)$ is the length two path $u,v,w$;
$P(v,w)$ is the counterclockwise path of length four.)  Edmonds'
algorithm maintains a data structure to calculate these paths
$P(x,b)$.  One reason the paths are needed is that they make up the
augmenting path found by the search. For example, in Figure 1, if an
edge from $B_2$ to a free vertex is added to the search graph it
completes an augmenting path that includes edges $a$ and $b$ and the
path joining them, $P(u,w)$.  A tree-based data structure that can be
used to compute a path $P(x,w)$ in time proportional to its length is
given in 

The paths $P(x,b)$ are also used to implement the expand step.
Suppose an expand step is done for an inner blossom $B$.  Before the
expand step \os. contains precisely two edges incident to $B$: an
unmatched edge leading to the parent of $B$ in \os. and a matched edge
leading to its unique child.  (In Figure 1 before an expand step for
$B_1$, these edges are $a$ and $b$.)  Let $x$ ($b$) be the vertex of
$B$ on the unmatched (matched) edge ($b$ is the base of $B$).  (In
Figure 1 these vertices are $u$ and $w$ of $B_1$, respectively.)  The
expand step replaces $B$ in \S.  by the subblossoms of $B$ along the
path $P(x,b)$.  (In Figure 1 these subblossoms are simply vertices,
but in general they can be large blossoms.) So in general an expand
step produces new outer blossoms and new inner blossoms. As mentioned
above, the new inner blossoms can be subsequently expanded.

\fi

Edmonds' algorithm finds an augmenting path 
$\o P$ in the graph $\oG$ that has
every blossom contracted. $\o P$ corresponds to
an augmenting path $P$ in the given graph $G$:
For any contracted blossom $B$ on an unmatched edge $xy$ ($x\in V(B)$) 
of  $\o P$,
$P$ traverses the path $P(x,\beta(B))$. If we augment the matching of $G$
along $P$,
every blossom becomes a blossom in the new matched graph:
For instance the above vertex $x$ becomes the new base of $B$. In Fig.\ref{1Fig}
if $\o P$ contains an unmatched edge $\alpha'$ that enters
$B$ at vertex $a$,
$P$ contains the subpath $P(a,\beta(B))$. The augment makes $a$ the base of $B$
as well as $B_1$;
in the contracted graph $\alpha'$ is the matched edge incident to $B$.

\subsection{Edmonds' weighted matching algorithm}
\label{EdAlgSec} 
For definiteness consider the problem of finding a maximum weight 
perfect matching.
The algorithm is easily modified for all the other variants of weighted matching. Without loss of generality assume a perfect matching exists.


The algorithm
is a primal-dual strategy
based on Edmonds' formulation of weighted matching as a linear program
(see the review in Appendix \ref{EdAppendix}).
It repeatedly finds a maximum weight
augmenting path and augments the
matching. The procedure to find one augmenting path is  a {\it
search}. If the search is successful, i.e., it finds an augmenting path
$P$, then an {\it augment step} is done. It augments the matching along
$P$. 
%The exact definition of unsuccessful search depends on the variant of
%the matching problem being solved and does not concern us here; see [L]. 
The entire algorithm consists of $n/2$ searches and augment steps.
At any point  in the algorithm
$V(G)$ is  partitioned into blossoms.
Initially every vertex is a
singleton blossom.




The following pseudocode gives a precise specification of the
search for an augmenting path; a more detailed discussion with examples follows.
Assume the graph has a perfect matching so this path exists.
For any vertex $v$, $B_v$ denotes the maximal blossom containing $v$.

% figure dimensions
\newlength{\figwidth}
\setlength{\figwidth}{\textwidth}
\addtolength{\figwidth}{-1in}
\newlength{\figindent}
\setlength{\figindent}{.5in}
\newlength{\vmargin}
\setlength{\vmargin}{.1in}
\begin{center}
  \fbox{
    \newlength{\Efigwidth}
    \setlength{\Efigwidth}{\textwidth}
    \addtolength{\Efigwidth}{-.3in}
\begin{minipage}{\Efigwidth}%{\figwidth}
\setlength{\parindent}{.2in}

\narrower{
\setlength{\parindent}{0pt}
\vspace{\vmargin}
\setlength{\parindent}{20pt}

\noindent
Repeat the following procedure until the search structure is a blossom
on vertex set $V$.

\smallskip
construct a maximal search structure of eligible edges in $S$

adjust dual variables in the search structure

}%narrower

\vspace{\vmargin}

\end{minipage}
}%fbox
\caption{Pseudocode for Edmonds' algorithm for critical matching with 
near-optimum duals.}
\label{EdAlgFig}
\end{center}
\end{figure}

make every free vertex or free blossom the (outer) root of an \os.-tree\;

{\bf loop}

\Indp

\If{$\exists$ tight edge $e=xy$, $x$ outer and $y\notin \S.$}
{\tcc{grow step}
let $\beta$ be the base of $B_y$, with $\beta\beta'\in M$\;
add $xy, B_y, \beta\beta', B_{\beta'}$ to \S.\;
}

\ElseIf{$\exists$ tight edge $e=xy$, $x,y$ outer in the same search tree, $B_x\ne B_y$}
{\tcc{blossom step}
merge all blossoms in the fundamental cycle of $e$ in \os.\;
}

\ElseIf{$\exists$ tight edge $e=xy$, $x,y$ outer in different search trees}
{\tcc{augment step}
\tcc{$xy$ plus the \os.-paths to $x$ and  $y$ form
an augmenting path $P$}
augment the matching along $P$ and end the search\;
}

\ElseIf{$\exists$ a nonsingleton inner blossom $B$ with $z(B)=0$}
{\tcc{expand step}


%update the matching on the edges of $B$

let \os. contain edges $xy$ and $\beta\beta'$ incident to $B$ where
$\beta$ is the base of $B$, $x\in V(B)$

let $B$ have subblossoms $B_i$

in \os. replace $B$ by the even length alternating path of subblossoms
$B_0,\ldots, B_k$ 

\goin that has $x\in B_0$, $\beta\in B_k$

\tcc{the remaining subblossoms of $B$ are no longer in \S.}



}

\lElse {adjust duals}

\bigskip

\caption{Pseudocode for a search in Edmonds' algorithm.}
\label{MAlg}
\end{algorithm}

A search constructs a subgraph $\cal S$. $\cal S$ is initialized
to contain every free blossom.
It is enlarged by executing three types of steps, called {\it grow},
{\it blossom},  and {\it expand steps} in 
\cite{G85b}. In addition the search changes the linear programming
dual variables in {\it dual adjustment steps}.
After a dual adjustment step, one or more of the other steps can be performed.
Steps are repeated until $\cal S$ contains the desired augmenting path.

$\cal S$ consists of blossoms forming a forest.
More precisely
if each blossom is contracted to a vertex, $\cal S$ becomes a
forest \os. whose roots are the free blossoms.
A blossom of $\cal S$ that is an even (odd)
distance from a root of \os. is {\it outer} ({\it inner}).
(The third possibility is a blossom not in $\cal S$.)
A vertex of $\cal S$
is outer or inner depending on the blossom that contains it. 
Any path from a root to a node in its tree of \os. is alternating.
So the matched edge incident to a nonroot outer blossom 
goes to its parent; the matched edge incident to an inner
blossom goes to its unique child.

In Fig.~1 suppose $B_0,\ldots,B_6$ are maximal blossoms,
edges $\gamma,\delta,\varepsilon$ are not part of \S.,
and blossom $B$ 
has not yet formed.
If $B_0$ is outer, the outer blossoms are the $B_i$ with $i$ even.
If a blossom step forms blossom $B$, the $B_i$ with $i$ odd change from
inner to outer.
Now we discuss the three steps that build up $\cal S$
(see also Fig. \ref{MAlg}).

\b

\noindent
{\bf Grow steps} 
A grow step enlarges \S..
It is executed for an edge $vx$ where vertex $v$ is outer and $x$ is
not in \S.. Let $x$ be in the maximal blossom $B$ with base vertex $\beta$.
$B$ is a matched blossom (by the initialization of \S.).
Let  $\beta\beta'$ be the corresponding matched edge.
$\beta'$ is the base vertex of a maximal blossom $B'$.
The grow step adds edge $vx$, 
$B$, edge $\beta\beta'$ and $B'$ to \S..
$B$ and
 $B'$ 
are new inner and
outer blossoms respectively.

In Fig.~1 if $\cal S$ contains outer blossom $B_0$ but no other $B_i$,
a grow step for edge $\alpha$ adds 
$\alpha, B_1$,  $(\beta(B_1),\beta(B_2))$ and $B_2$ to $\cal S$.
Two more grow steps add the
other $B_i$, $i=3,\ldots,6$.

\b

\noindent
{\bf Blossom steps} 
A blossom step is executed for an edge $e$ that joins two distinct
outer blossoms in the same tree of \os..
It combines all blossoms along the fundamental cycle
of $e$  to form a new
blossom $B$. Note that $B$ is outer: In proof let $A$ be the blossom
closest to the root in $e$'s fundamental cycle. $B$ is outer if $A$ is.
If $e$ is incident to $A$ then 
$A$ is outer, by definition. If $e$ is not incident to $A$ then
the ends of $e$ descend from 2 distinct children of $A$.
$A$ must be outer, since as previously noted any inner blossom has only
one child. 

In Fig.~1 suppose $\cal S$ contains blossoms $B_i$, $i=0,\ldots,6$,
with $B_i$ outer for $i$ even.
A blssom step for $\gamma$ would form blossom $B$.
Alternatively the search
might do a blossom step for $\varepsilon$, then later one for $\delta$,
and still later one for $\gamma$. Other sequences are possible, and the one
executed 
depends on the costs of these edges.

\b

\noindent
{\bf Expand steps} 
An expand step replaces an inner blossom $B$ of $\cal S$ by some of its
subblossoms. Specifically let
$B$, with
base vertex $\beta$, be  incident to
edges $xy$ and 
$\beta\beta'$
in \os., with $x\in V(B)$.
Let $x$ ($\beta$) be in the maximal subblossom
$B_0$ ($B_r$) of $B$, respectively, and let $P(B_0,B_r)$ be
the even-length alternating path formed from  edges of $B$.
Then $B$ is replaced by  $P(B_0,B_r)$ in \os.. The remaining
subblossoms of $B$ are no longer in \os. -- they are now eligible
to enter \os. in grow steps.
\os. remains a forest.
 
In Fig.~1 when $\cal S$ contains all blossoms $B_i$,
an expand step for $B_1$ replaces it by
vertices $a_0,a_1,$ blossom $A$, $a_3$, and  $a_4$.
The other two subblossoms of $B_1$ leave \os..

\b

This completes the description of the three steps that construct \S..
Note that once a vertex becomes outer it remains 
in $\cal S$ and outer for the rest of the search.
In contrast vertices
can alternate between being inner  and 
not being in $\cal S$ (perhaps ultimately becoming outer in a grow
or blossom step).
This alternation can occur $\Theta(n)$ times for a given vertex $v$
in one search
(the upper bound  $n$  holds since each time $v$ is
involved in an expand step, the size of the maximal blossom containing $v$
decreases). 

The sequence of steps executed by the search depends on
the costs of edges and the values of the dual variables. The algorithm
executes a given step when a corresponding edge becomes {\em tight},
i.e., its dual variables satisfy
the complementary slackness conditions of linear
programming. For example in Fig.~1 the blossom step for $\gamma$ is done
when $\gamma$ becomes tight. The dual adjustment step modifies dual
variables so that additional edges become tight and corresponding grow,
blossom or expand steps can be done.
The dual adjustment step involves finding a candidate edge 
that is closest to being tight, and then changing the dual variables to make it
tight. It is given in detail in Appendix \ref{EdAppendix}.

The search terminates in an augment step.  It is executed for an edge
$e$ that joins 2 different trees of \os..  Let $e$ join blossoms $X_0$
and $X_1$, with $X_i$ in the tree rooted at free blossom $B_i$.  $e$
plus the edges of \os. from $X_i$ to $B_i$ forms an augmenting path
$\o P$ in the current contracted graph $\oG$.  We augment the matching
along the path $P$ in $G$, as described above. 
This changes base vertices of various
blossoms on $\o P$ as well as $P$.

After an augment the algorithm halts if every vertex is matched.  
Otherwise the next search is initialized: Every free blossom is made a
tree root of \S.. Then we proceed as above.
Note that the initialization retains all the blossoms --
a maximal blossom that is not free is now a blossom not in \S..%
\footnote{This contrasts with maximum cardinality matching,
where initialization discards the blossoms.
As a result there are no inner blossoms.}

\b


\noindent
{\bf Data structure for blossoms}
The data structure consists of two  parts,
both  used in most implementations of Edmonds' algorithm. 
The maximal outer blossoms are tracked 
using
a data structure for set-merging.
It suffices to use 
an algorithm that executes $O(m)$  
$finds$ and $O(n)$ $unions$ in a universe of $n$ elements in
 $O(m+n\log n)$ total time and $O(n)$ space
(e.g., the  simple relabel-the-smaller-set algorithm ~\cite{AHU, CLRS}).  
The incremental-tree set-merging algorithm of 
Gabow and Tarjan \cite{GT85} improves this to linear time.
The set-merging data structure is used to manipulate the
vertices of \os., e.g., a blossom step does 
$finds$ 
to identify the outer vertices in
the fundamental cycle in $\o G$
and $unions$ to  contract the cycle.
(The inner vertices are identified using the algorithm of Appendix \ref{GrowExpandSection},
as discussed at the start of Section \ref{BMergingSec}.)

 
The second part of the data structure
%This data structure 
is based on  a forest representing
the laminar family of blossoms.
The main use is to compute
$P(x,\beta)$ paths. These paths are used to find  augmenting paths,
and to compute the supporting forest for tree-blossom-merging
(Section \ref{TSec}).
The data structure is also used 
in expand steps to update \os..

The laminar family is defined as follows.
Every maximal blossom 
$B^*$ has a corresponding tree $T(B^*)$.
The root of $T(B^*)$ is a node corresponding to $B^*$ and the leaves
correspond to $V(B^*)$.
The children of any node $B$ are the
subblossoms $B_i$ of  $B$.
$T(B^*)$ is an ordered tree,
with 
the children $B_i$ of $B$ ordered according to
the edges of $B$ that form a cycle spanning the  contracted
$B_i$ (in Definition \ref{BlossomDefn} these are the edges
of the two paths $P(X_i,Y)$ plus $X_0X_1$). 

The data structure for the laminar family has the following components. 
The root node (for $B^*$) records the vertex $\beta(B^*)$.
The children
of any node $B$ form a doubly linked ring. Each link also records the
edge $xy$ of $G$ ($x,y\in V(G)$) that joins  the two subblossoms.
Finally  $T(B^*)$ has parent pointers.
Additionally we assume the edges of the matching $M$ are marked as such.


This data structure has size $O(|V(B^*)|)=O(n)$.
In proof the
leaves of the tree form the set $V(B^*)$.
Each interior node is a nonsingleton blossom, so
there are fewer than $|V(B^*)|$ interior nodes.

The data structure is initially constructed in the blossom step.
The expand step involves replacing the inner node $B^*$ with
a path formed from the children of $B^*$. The other applications are
based on  $P(x,\beta)$ paths.
For completeness we give a routine for computing these paths.

We start with
some simple primitive operations.
Given $x\in V(B^*)$ the blossoms containing $x$ are identified by
tracing the  path from the leaf $x$ to the root of $ T(B^*)$.
An interior node $B\ne B^*$ with a link corresponding to
edge $xy\in M$, $x\in V(B)$
has base vertex $x$. 
If neither link from $B$ is matched then 
the base vertex of $B$ is  that of its first ancestor 
having an incident matched edge.

We turn to computing the $P(x,\beta)$ paths.
The main algorithm requires
$P(x,\beta)$ in the form of a list of edges, say $L$.
The supporting forest requires this list to be ordered
as an $x\beta$-path.
The following recursive routine uses a global list $L$.
Each recursive invocation enlarges $L$ with the appropriate edges.
 
Consider any blossom $B$ (maximal or not) and a vertex $x\in V(B)$.
The recursive routine adds the edges of $P(x,\beta(B))$
or its reverse to $L$.
%We use a recursive routine based on (\ref{PvbEqn}).
The routine is called with 4 %four %5 
arguments: 

\bigskip

{\narrower

{\parindent=0pt

vertex $x$ and the child $B_0$ of $B$ that contains $x$;

the base vertex $\beta(B)$; % and the child $B_k$ of $B$ that contains $\beta(B)$;

a bit $r$ equal to 1 if the reverse path
 $P(\beta(B),x)$ is desired, else 0.

}
}


\bigskip

The following procedure is used if $r=0$:
First consider the general case $B_0\ne B_k$.
Starting at $B_0$ follow links to the siblings $B_i$ corresponding
to the blossoms of (\ref{PvbEqn}).
The last blossom $B_k$ is identified as the node whose two links
both have unmatched edges.
For each $B_i$ use a recursive call to find the 
corresponding subpath of (\ref{PvbEqn}), and then for $i<k$ add the edge
corresponding to the link leaving $B_i$
(i.e., $\beta_i \beta_{i+1}$ or $x_i x_{i+1}$) to $L$.
The arguments for each recursive call 
$P(x_i,\beta(B_i))$ are easily found using the above primitives,
with the value of $r$  corresponding to (\ref{PvbEqn}).
(The argument $\beta(B_i)$ is known from the matched edge incident
to $B_i$, for any $i<k$. For $i=k$ it is known from the 
matched edge incident to an
ancestor of $B$, unless $\beta(B)=\beta(B^*)$. That base is explicitly
recorded in the data structure.) 
The base case $B_0=B_k$ is handled as in the definition of
$P(x,\beta)$, i.e., immediately return if
$B_0$ is a vertex else  recurse as above.

Now suppose the routine is called with $r=1$.
The base case is unchanged. For the general case first find
which of the two links from $B_k$ corresponds to an edge on the desired path.
Do this by
following  links from $B_0$ to $B_k$, starting with the appropriate link from
$B_0$.  Then follow links from $B_k$ to $B_0$, starting with the appropriate link. As in the $r=0$ case, issue recursive calls, and for $i>0$ add the
edge leaving $B_i$.
The recursive calls have $r$  set to
the complement of the bit corresponding to (\ref{PvbEqn}).


The arguments for the initial call to find $P(x,\beta(B))$
are found as above.

Regarding efficiency first observe that 
the procedure is easily implemented to use time $O(|V(B)|)$, as follows.
For any recursive call
$P(x_i,\beta(B_i))$ the path-tracing to find the subblossom containing
$x_i$ is only done the first time it is needed.
Once the path is known it is treated like a stack to get
subsequent subblossoms containing $x_i$.

The time can be improved to $O(|P(x,\beta(B))|)$.
This requires eliminating part of the path-tracing to find the blossoms
containing $x_i$. Specifically we must skip over the smallest blossoms 
containing $x_i$ as base vertex, since they do not contain any edge of
the output  $P(x,\beta(B))$.
To accomplish this we augment the data structure 
so each matched edge corresponding to a link in $T(B^*)$ 
has a
pointer to that link.
The path-tracing 
for $x_i$ starts at the link for the matched edge incident to $x_i$.
This bypasses all the unwanted blossoms
with base vertex $x_i$.

\iffalse
$P(x_i,\beta(B_i))$ the path-tracing to find the subblossoms containing
$x_i$ and $\beta(B_i)$ need only be done the first time they are needed.
Once the path is known it is treated like a stack to get
subsequent subblossoms.
\fi

\iffalse
it is easy to see the time is  linear
in the size of  the subtree of $B$ in $T(B^*)$.

The time for this procedure is linear in its length, 

$O(|V(B)|)=O(n)$.
In proof it is easy to see the time is  linear
in the size of  the subtree of $B$ in $T(B^*)$.
The leaves of this subtree form the set $V(B)$.
Each interior node is a nonsingleton blossom, so
there are fewer than $|V(B)|$ interior nodes.
\fi




\subsection{The blossom-merging problem}
\label{BMergingSec} 
This completes the sketch of Edmonds' algorithm.
Our task is to implement a search in time $O(m+n\log n)$.
It is known how to implement most parts
within the desired time bound. For dual adjustment steps
a Fibonacci heap $\cal F$ is used. It contains the candidate edges
for tightness
mentioned above. The heap minimum gives the next edge to be made
tight. This is analogous to Fredman and Tarjan's
implementation of Dijkstra's algorithm
by Fibonacci heaps 
and uses the same time per search, 
$O(m+n\log n)$. 
Dual variables are maintained in time $O(n)$ per search using
offset quantities (e.g., \cite{GMG}).
The processing associated with grow and expand steps can be done in time 
$O(m\alpha(m,n))$ using a data structure for list splitting given in 
Gabow \cite{G85b}.%
\footnote{After the conference version of this paper
the time for  list splitting was improved 
by Pettie \cite{Pettie} and Thorup \cite{Thorup}.}
A simpler algorithm is presented in Appendix \ref{GrowExpandSection}; it suffices for our time bound and makes this paper self-contained.
The current blossom containing a given vertex is found using
the set-merging data structure of last section
for  outer vertices and the grow/expand algorithm for nonouter vertices.
Finally note after a successful search,
the corresponding augment step can be done in time $O(n)$ using the $P(x,\beta)$ paths
 \cite{G76}. 
This leaves only the blossom steps: implementing the blossom steps of a 
search in time $O(m+n\log n)$ gives the desired result.
(This observation is also made by Gabow, Galil, and Spencer\cite{GGS}.)

The problem of implementing the blossom steps of a search
can be stated precisely as the {\it blossom-merging problem} 
which we now define. (\cite{GGS} defines a similar problem called 
on-line restricted component merging, solving it
 in time  $O( m \log  \log  \log_{2+m/n} n  +  n \log n)$.)
The universe consists of a graph with vertex set $\cal O$ and edge set $\cal E$,
both initially empty.
($\cal O$ will model the set of outer vertices, $\cal E$ the set of edges joining
two $\cal O$-vertices and thus candidates for blossoms.)
At any point in time $\cal O$ is partitioned into
subsets called blossoms.
The problem is to process (on-line) a sequence of the following types
of operations:

\iffalse
At any point in time \E. contains
all edges that join two outer vertices in theEdmonds' algorithm. 
Thus $\cal E$ includes all edges that can cause blossom steps.
(\E. also contains edges that join two outer vertices in the same
blossom. Such an edge is no longer relevant.)
\fi

\b

\long\def\twolines #1 #2{\vtop{\hbox{#1}\hbox{#2}}}


{%\parindent=40pt

{%\narrower

%\parindent=0pt

$make\_blossom(A)$ -- \twolines
{add the set of vertices $A$ to $\cal O$ and make $A$ a blossom}
{(this assumes $A\cap {\cal O}=\emptyset$ before the operation);}

\smallskip



$merge(A,B)$ -- \twolines {combine blossoms $A$ and $B$ into a new blossom} 
%called $B$
{(this destroys the old blossoms $A$ and $B$);}

\smallskip

$make\_edge(vw, t)$ -- %\twolines 
{add edge $vw$, with cost $t$, to $\cal E$}
(this assumes $v, w\in O$);

\smallskip

\fm. -- \twolines {return an edge $vw$ of $\cal E$ that has minimum cost
subject to the constraint} 
{that $v$ and $w$ are (currently)
in distinct blossoms.}

}}


\b

Let us sketch how these four operations are used to implement 
a search. Grow, expand 
and blossom steps each create new outer blossoms. They perform
$make\_blossom$ operations to add the new outer vertices to $\cal O$. They also
perform $make\_edge$ operations for the new edges that join two 
outer vertices. For example in Fig. \ref{1Fig}
if $B_0$, $B_5$ and $B_6$ are in $\cal S$
and a grow step is done for edge $\alpha$ then
$make\_blossom(B_2)$ is done; also
$make\_edge$ is done for edge $\delta$. Note that in $make\_edge(vw,t)$, 
$t$ is not the given cost $c(vw)$. 
Rather $t$ is $c(vw)$ modified by dual values; 
this modification allows the algorithm to make dual adjustments efficiently
(see e.g., Gabow, Micali, and Galil\cite{GMG}). The value of $t$
is unknown until the time of the $make\_edge$ operation. From now
on, since we are only concerned with the blossom-merging problem,
the ``cost'' of an edge of $\cal E$ refers to this value $t$, not the
cost input to the matching algorithm.

A blossom step performs $merges$ to construct the new
blossom. In Fig.~\ref{1Fig} the operations
{\it merge}$(B_i,B_0)$, $i=1,\ldots, 6$ construct $B$.
Note that information giving the
edge structure of blossoms is maintained and used in the
outer part of the algorithm -- 
it is not relevant to the blossom-merging problem. For this problem
a blossom $B$ is identical to its vertex set $V(B)$;
the $merge$ operation need only update the information about the
partition of $\cal O$ induced by blossoms. Also in the blossom-merging problem 
``blossom'' refers to a set of the vertex partition, i.e., the result
of a $make\_blossom$ or $merge$ operation. 
The latter may be only a
piece of a blossom in Edmonds' algorithm (as in the 6 merges above)
 but this is not relevant.



A \fm. operation
is done at the end of each of the three search steps.
 The returned edge,
say $e$,
is used in the above-mentioned Fibonacci heap $\cal F$
that selects the next step of the search.
Specifically $\cal F$ has one entry that maintains the smallest
cost edge of $\cal E$. If that entry already contains $e$
nothing is done. If the entry contains an edge of larger cost than $e$,
the entry is updated to $e$ and a corresponding $decrease\_key$ is done.
The smallest key in $\cal F$ (which may or may not be the key for $e$)
is used for the next dual adjustment and the next step of the search.

\iffalse
In Fig. \ref{1Fig} if $\delta$ is  returned by {\it find\_min}
it gets added to $\cal F$.
For correctness of the implementation
it is important that the blossom-merging problem uses
a {\it find\_min} operation
rather than {\it delete\_min}: The current
minimum edge $e$ for a future blossom step 
may not be selected (in the dual adjustment step) as the next tight
edge for Edmonds' search algorithm. A different edge $e'$ may be
selected. The next step of the search, for $e'$,
may create new blossom steps for edges smaller than $e$.
So it would be premature to delete $e$ from the blossom-merging data
structure when it is found to be minimum.
\fi

To illustrate this process in 
Fig.\ \ref{1Fig} suppose $\cal O$ consists of 
$B_i$ for $i=0,1,2,5,6$ and $\cal E=\{\delta,\varepsilon\}$.
Furthermore  the entry in $\cal F$ contains edge $\delta$.
A grow step for $B_3$ and $B_4$ adds $V(B_4)$ to $\cal O$ and
 $make\_edge$  
is done for $\gamma$. If $\gamma$ is now the smallest edge in
$\cal E$, 
the entry in \F. for the next blossom step changes from
$\delta$ to $\gamma$ and a corresponding {\it decrease\_key} is performed.


Our task is to implement a sequence of these 
operations: $make\_blossoms$ adding a total of $\le n$ vertices,
$\le m$ $make\_edges$, $\le n$ $merges$ and $\le n$ \fms.,
in time $O(m+n\log n)$. The bound on \fms. follows since
\fm. need not be done after an expand step that does not create a
new outer vertex (e.g., in Fig.~\ref{1Fig} with blossom $B_1$ already
expanded,
expanding $A$ does not add outer vertices).
Every other step creates a new outer vertex
(a blossom step changes an inner vertex to outer). So
there are at most $n$ such steps and $n$ corresponding \fms..

The difficulty in solving the blossom-merging problem is
illustrated by Fig.~\ref{1Fig}. When each $B_i$, $i=0,\ldots, 6$ is a
blossom, edges  $\gamma, \delta, \epsilon$ are candidates
for \fm.. If a blossom step for $\gamma$ is done, 
$\delta$ and $\epsilon$
become irrelevant -- they  no longer join distinct blossoms.
If we store the edges of $\cal E$ in a priority queue
 useless edges like $\delta, \epsilon$ 
can end up in the queue.  
These edges 
eventually get deleted from the queue but the deletions 
accomplish no useful work. The time bound 
becomes $\Omega(m\log n)$.
(This also indicates why 
there is no need for a {\it delete\_min} operation in the 
blossom-merging problem: If edge $\gamma$  gets returned by
\fm. and as above
a blossom step forms $B$, edge $\gamma$ becomes  irrelevant.)
% is used to do a blossom step, after the blossom step $x$ and $y$ are in
% the same blossom; hence $xy$ is not irrelevant
% for subsequent {\it find\_mins}).

\section{Tree-blossom-merging}
\label{TSec}
Tree-blossom merging incorporates 
the topology  of the search graph
into general blossom-merging, in two ways.  This section starts by defining the
tree-blossom-merging problem and showing
how it can be used to implement the blossom
steps of Edmonds' algorithm. Then it presents our 
tree-blossom-merging algorithm.


The first goal is to maintain a representation of the search graph $\cal S$ by a
forest that changes as little as
possible.  We cannot avoid adding nodes, e.g., in grow steps.
But we can define a forest that does not change in expand steps.
Consider a search tree, i.e., a tree \ot. in the forest \os..
 
\begin{definition}
\label{STreeDefn}
A tree $T$ {\em  supports the search tree \ot.}
if each blossom $B$ of \ot. has a corresponding
subtree $T_B$ in $T$, these subtrees partition 
the vertices of $T$ and are joined by  edges of \ot., and 
for each blossom $B$:

\case{$B$ is outer} Let $B$ have  base vertex $\beta$.  $V(B)=V(T_B)$. 
% and $T_B$ is rooted at $b$.
If $B$ is incident to the matched edge $\beta\beta'$ in \ot.
 then $\beta'$ is the parent of $\beta$
in $T$. If $B$ is a free vertex then $\beta$ is the root of $T$.

\case{$B$ is inner} Let $B$ be  incident to edges $vx, \beta\beta'$ 
in \ot., where $x,\beta\in V(B)$ and $\beta\beta'$ is matched. Then
$T_B$ is the path $P(x,\beta)$ and $v$ is the parent of $x$ in $T$.
\end{definition}

Take any vertex $v$ in an outer blossom $B$ of \ot..
$v$ has a path to the root in both \ot. and $T$,
say $p_{\ot.}(v)$ and $p_T(v)$ respectively. 
Let
$p_{\ot.}(v)=(B_0=B,B_1,\ldots,B_k)$.
$p_T(v)$ consists of subpaths through each subtree $T_{B_i}$.
For even $i$ the subpath 
contains the base vertex
$\beta(B_i)$ and perhaps other $B_i$-vertices. 
For odd $i$ %, $B_i$ is inner, and 
the subpath is 
the entire path $T_{B_i}$.
This correspondence will allow us to track potential blossom steps,
as well as
execute them,
in the supporting forest. % rather than \os..

\iffalse
an edge joining two outer blossoms  
the blossoms in 
If $vw$ is an edge joining outer vertices $v$ and $w$,
the nearest common ancestor of  $nca(v,w)$ in $T$
is in the blossom 
the blossom $A$ closest to the root
in the fundamental cycle of $xy$ in \os. 
So we can decide which the next blossom
the set of potential blossom steps can be we can use $T$ can be used
to determine the next blossom step of the algorithm.

is the blossom base verte
whose base vertex has $\beta(A)$ $nca(x,y)$
\fi

We
will maintain
the supporting tree $T$ 
using this operation:


%as the algorithm modifies \os. 

\b


{%\parindent=40pt

%\narrower

\alm$(x,y)$ -- add a new leaf $y$, with parent $x$, to  $T$.

}

\b

\noindent
Here we  assume
$x$ is a node already in $T$ and $y$
is a new node not in $T$. We also assume the data structure for $T$
records parent pointers created by \alm.



We now show how $T$ is maintained
as the search algorithm executes
grow, blossom and expand steps. 
Assume the partition of $V(T)$
into outer blossoms and individual 
vertices in inner blossoms
is maintained by a set-merging algorithm.



\iffalse
We show how to update $T$ using $add\_leaf$ operations to obtain a
tree supporting the new search graph.  
\fi


Suppose a grow step enlarges $\cal S$ by adding
unmatched edge $vx$, inner blossom $B$, matched edge 
$\beta\beta'$ and 
outer blossom $B'$,
where vertices $v\in V(\ot.)$, $x, \beta\in B$ and $\beta'\in B'$.
First compute $P(x,\beta)$ and write it as 
$x_i,\ i=0,\ldots, k$ where $x_0=x$, $x_k=\beta$.
Enlarge $T$ by performing 
\alm$(v,x_0)$, \alm$(x_i,x_{i+1})$ for $i=0,\ldots, k-1$,
\alm$(x_k,\beta')$ and finally
\alm$(\beta',w)$ for every $w\in B'-\beta'$.
Merge the vertices of $B'$ into one set.
(The search algorithm accesses the vertices of $B'$ from
the blossom data structure 
at the end of Section \ref{EdAlgSec}.)

Consider a blossom step for edge $vw$.  It combines the blossoms on
the fundamental cycle $C$ of $vw$ in \ot..  Let blossom $A$ be the
nearest common ancestor of the blossoms containing $v$ and $w$ in
\ot..  $A$ is an outer blossom.  $C$ consists of the subpaths of
$p_{\ot.}(v)$ and $p_{\ot.}(w )$ ending at $A$.  
In $T$, merge every
outer blossom in $C$ into the blossom $A$.  
For each inner blossom $B$ in $C$, 
do \alm$(v,u)$ for every vertex $u\in B-V(T)$.
Then merge every vertex of $B$ into $A$. 
The new blossom $A$ has the correct subgraph $T_A$ 
so the updated $T$ supports \ot..

\iffalse
The former
corresponds to the subpath of $p_T(v)$ ending at $\beta(A)$, and similarly
for the latter. 

 belonging to an inner blossom of $C$, unless $u$ is
already
in $T$.  Perform the corresponding merges into blossom $A$.  
\fi


Lastly consider an expand step. 
The expand step in the search algorithm
replaces an inner blossom $B$ by the subblossoms along the
path $P(x,\beta)$, say subblossoms $B_i$, $i=0,\ldots,k$,
where $x\in B_0$ and $\beta\in B_k$.
By definition $T_B$ is 
the path $P(x,\beta)$.
For odd $i$, $B_i$ is a new outer blossom of \ot.. 
Perform \alm$(\beta(B_i),v)$
for every vertex $v\in B_i-V(T)$.
Merge the vertices of $B_i$.

For correctness note that
for even $i$, $B_i$ is a new inner blossom of
\ot.. 
Equation
(\ref{PvbEqn}) gives the subpaths of $P(x,\beta)$ through the $B_i$.
$T$ contains the path $P(x_i,\beta(B_i))$, and $x_{i-1}$ is the parent
of $x_i$. 
\iffalse
(This is clear if $B$ was made inner in a grow step.
The other possibility is that $B$ became inner in an expand step.
In that case we use a simple induction.)
\fi
So $T_{B_i}$ satisfies Definition \ref{STreeDefn}  as required.



\iffalse
p(x,b)= p(x,b_0), p(b_1,x_1),p(x_2,b_2),p(b_3,x_3),\ldots,
p(x_k,b_k).
\end{equation}
Here $b_i$ is the base vertex of $B_i$.
$x_i$ is the vertex of $B_i$ on the unmatched edge of $A$ incident to $B_i$.
For odd $i$, $p(b_i,x_i)$ is the reverse of path $p(x_i,b_i)$. 
\fi

This completes the algorithm to maintain $T$.
It is easy to see the total time in maintaining $T$ is $O(n)$, since
$P(x,\beta)$ paths are computed in time
linear in their size.

\iffalse
\begin{lemma}
In a search of Edmonds' algorithm a forest supporting the trees
of \os. can be maintained
in time $O(m+n)$.
\end{lemma}

\begin{proof}
The incremental-tree set-merging algorithm of 
Gabow and Tarjan
\cite{GT85} maintains the partition of $V(T)$ into maximal blossoms
in linear time.
(Note this lemma only concerns the time spent 
creating and maintaining the supporting forest.
For instance no time is spent in an expand step when a new inner
blossom
$B_i$ is formed. All the processing associated with $B_i$ is accounted
for in the time bound for expand steps.) 
\end{proof}


We incorporate the algorithm to maintain the supporting forest
into a search of Edmonds' algorithm. Using the algorithm of Section \ref{NCASec}
the time for \al. is $O(1)$, so the time for a search
increases by only $O(n)$. 
\iffalse
This follows since using a data
structure such as  \cite{GMG} mentioned above,
the algorithm finds the vertices to be added to
$T$ in time linear in their number. 
\fi
\fi

\iffalse
The supporting tree is updated for a blossom step
the same way as the search forest \os.
(with the minor addition that new vertices are added for 
previously inner blossoms).
So our algorithm for the blossom-merging problem can
\fi





\iffalse
Even using  a supporting forest
the blossom-merging problem seems difficult. 
\fi


As mentioned the correspondence between paths $p_T$ and $p_{\ot.}$
allows us to track 
potential blossom steps in the supporting forest.
This still appears to be challenging.
Our second
simplification of the problem is to assume
$make\_edge$ adds only  back edges, i.e., edges joining
a vertex to some ancestor.
Clearly
 a blossom step for an edge $vw$
is equivalent to blossom steps for the two
edges $va$ and $wa$, for $a$ the nearest common ancestor of
$v$ and $w$ in $T$. So we can
replace $vw$ by these two back edges.

To accomplish this reduction we use a data structure for dynamic
nearest common ancestors. Specifically the algorithm maintains a tree 
subject to two operations.
The tree initially consists of a dummy root \rt, and
it grows using \alm\ operations. The second operation is

\b

{%\parindent=40pt

{%\narrower

$nca(x,y)$ -- return the nearest common ancestor of vertices $x$ and $y$.

\iffalse
$nca(x,y)$ -- \vtop{
\hbox{return the nearest common ancestor of vertices $x$ and $y$}

\hbox {(if $x$ and $y$ are in 
different trees, return $\emptyset$).}
}
\fi

}
}

\b



In summary we implement  Edmonds' algorithm as follows.
The search algorithm constructs 
supporting trees for the trees of \os.
using \al. operations. (Each supporting tree is rooted at a child of
\rt.)
%As part of this operation, 
%each vertex $y$ records its depth $d(y)$ in
%$T$ (we use it in the next section). 
When the search discovers an edge $vw\in E$
joining two outer vertices, it
performs $nca(v,w)$ to find the nearest common ancestor $a$.
If $a=\rt$ an augmenting path has been found.
Otherwise the search algorithm
executes the blossom-merging operations
$make\_edge(va,t)$ and $make\_edge(wa,t)$ for appropriate $t$. 

Each grow, blossom, and expand step performs all the appropriate 
$make\_edges$, and concludes with a 
\fm. operation. Assume this operation returns
back edge $va$, corresponding to edge $vw\in E$.
Assume neither $va$ nor  $wa$ has been 
previously returned.
As mentioned above, 
the Fibonacci heap \F. records edge $vw$ as the smallest candidate 
for a blossom step. If $vw$ is selected for the next step of the search algorithm, the corresponding blossom step is performed. Also blossom-merging $merge$ operations are
executed to form the new blossom in the supporting tree. These operations
place
$v$ and $w$ in the same blossom of the supporting tree. So 
$wa$ will never be returned by future 
\fms. (by definition
of that operation).

Let us estimate
the extra time that these operations add to a search
of Edmonds' algorithm.
The algorithm for maintaining the  supporting tree $T$
uses the incremental-tree set-merging algorithm of  Gabow and Tarjan \cite{GT85}
for $merge$ operations. It
maintains the partition of $V(T)$ into maximal blossoms
in linear time.
The dynamic nca algorithm of \cite{G90, G17} uses  $O(n)$ time for
$n$ \al. operations and $O(m)$ time for $m$ $nca$ operations.%
\footnote{After the conference version of this paper
Cole and Hariharan \cite{CH}
used a similar approach to allow these and other dynamic nca 
operations. In addition their time bounds are
worst-case 
rather than amortized.}
So excluding the time for $make\_edges$ and \fms.
the extra time is $O(m+n)$. 



We have reduced our task to solving the
{\it tree-blossom-merging problem}. It is defined on a tree $T$
that is constructed incrementally by \al. operations.
Wlog assume the operation
\alm$(x,y)$ 
computes $d(y)$, the depth of vertex $y$ in its supporting tree.
There are three other operations, $make\_edge$, $merge$ and \fm.,
defined as in the blossom-merging problem with the restriction that
all edges of $\cal E$, i.e., the arguments to $make\_edge$, are back edges.

There is no $make\_blossom$ operation -- we assume Edmonds'
algorithm does the appropriate 
\al. and $merge$ operations.
Note that \E. is a multiset:
A given edge $vw$ may be added to \E. many times
(with differing costs) since although an edge $uv\in E$ will become
eligible for a blossom step at most once, different $u$ vertices can
give rise to the same back edge $vw$.
\iffalse
for instance uv and u'v may both add vw to \E., a blossom step may be done
for uv. later a blossom step may be done for u'v
this makes vw irrelevantto the tree-blossom data structure, but not u'w
\fi
Our notation assumes
the edges of \E. are directed towards the root, i.e., $vw\in \E.$ has
$d(v)>d(w)$. %(Recall $d$ denotes depth in the supporting tree.)

As before for any vertex $x$,  
$B_x$ denotes the blossom currently containing $x$.
Assume that the $merges$ for a blossom step
are performed in the natural bottom-up order, i.e.,
for $vw\in \E.$ the search algorithm
traverses the path in \os. from $B_v$ to $B_w$, repeatedly
merging (the current) $B_v$ and
its parent blossom.
In tree-blossom-merging
we call any set resulting from  a $merge$ operation
a ``blossom'' even though it need not be a blossom of Edmonds' search algorithm.

\iffalse
Let us prove that this implementation of Edmonds'
algorithm is correct. The main observation is that
an edge $vw$ in the given graph joins two distinct outer blossoms
if and only if at least one of its corresponding 
edges $va$, $wa$ in $\cal E$ joins two distinct blossoms.
This observation holds by Lemma 2.1. 
The observation shows that $find\_min$ returns (a back edge corresponding to)
the desired minimum edge. Thus the implementation is correct.

Section \ref{NCASec} shows that the total time for $O(n)$ \al. operations and 
$O(m)$ $nca$ operations is $O(m+n)$.
\fi


\iffalse
\subsection{The simple merging algorithm.}
\label{SimpleAlgSec} 
This section gives an algorithm for tree-blossom merging
that uses $O(m+n\log^2n)$ time and $O(m+n\log n)$ space. 
This implements a search of Edmonds' algorithm 
in the same resources.

The fact that tree $T$ is constructed incrementally is not central to
our merging algorithms. (Of course it is important in Section 3.)
The algorithms use 
only a simple representation of $T$: each vertex $x$ in $T$ records its
parent and its depth $d(x)$ in $T$. 
It is a simple matter to record these values in total time
$O(n)$: The operation $add\_leaf(x,y)$ computes the values for
$y$ from those of $x$. 

For a set of edges $S$, define $smallest(S)$ as an edge in $S$ with
smallest cost. If several edges tie for smallest cost, 
$smallest(S)$
can be chosen from amongst them arbitrarily (so $smallest(S)$ always
denotes one edge). If $U$ and $U'$ are disjoint sets of 
vertices then $smallest(U,U')$ is defined similarly, referring
to the edges of $\cal E$ from $U$ to $U'$. 
Note that if $B$ is a blossom, for any vertex $v$
it suffices for the algorithm
to retain one edge $smallest(B,v)$ -- all other edges from $B$ to $v$
can be discarded, since they need never be returned as the value of
$find\_min$.

The data structure has three main parts: a priority queue ${\cal F}_0$, 
a data structure for edges and a data structure for blossoms. We describe each
in turn. Several Fibonacci heaps are used. We make the convention of
using an edge $e$ to represent a key in these heaps. Strictly speaking
the key is the cost of $e$,
but $e$ is stored in the heap anyway; no confusion will result.

The priority queue ${\cal F}_0$ 
keeps track of the smallest blossom step edge incident to each blossom.
More precisely ${\cal F}_0$  is a Fibonacci heap, with an entry for each
blossom $B$. The entry for $B$ is $smallest(B,O-B)$.
Thus a {\it find\_min} operation in our data structure amounts to
a Fibonacci heap {\it find\_min} in ${\cal F}_0$.
% A $make\_edge$ operation can decrease the key for a blossom in ${\cal F}_0$; 
% a $merge$ operation deletes entries. The processing associated with
% ${\cal F}_0$ uses time $O(m+n\log n)$.

To define the edge data structure, say that the {\it rank} of an 
edge $vw\in {\cal E}$ equals
\[\f{\log |d(v)-d(w)|}.
\]
Thus the rank of an edge is between zero and $\f{\log(n-1)}$.
The edge data structure is a partition of ${\cal E}$ into sets called packets.
% 
% with the vertex of greater depth, say $v$. Thus each outer vertex $v$
% has a set of back edges in $\cal E$.
% This set is partitioned into at most $\log n$ subsets, which we call 
% \footnote *{
% 
% Recall that $d(v)$ denotes the depth of vertex $v$ in $T$.
The {\it packet of rank $r$ for vertex $v$} contains all edges 
$vw\in {\cal E}$ with rank $r$ and $d(v)>d(w)$.
A packet $P$ is implemented as a linked list of edges; it also records 
%the packet rank $r$ and 
$smallest(P)$.
Each vertex $v$ has an array $packet_v[0..\f{\log n}]$ of
pointers to its packets, i.e., $packet_v[r]$
points to the packet of rank $r$ for $v$.
Observe that a given edge can be added to the appropriate packet in $O(1)$ 
time.
% The extra space for the packet pointers is $O(n\log n)$ total.
(This notion of packet is similar in spirit, but not detail, 
to the data structure of the same name in \cite{GGS, GGST}.)

To {\it open a packet} $P$ means to transfer the edges of $P$
into the rest of the data structure. This destroys $P$, i.e., a packet
is opened only once. 
%
%Each packet is marked open or not.
%
It is useful to be able to restrict the $smallest$ function to
edges coming from opened packets -- for this we use the function 
$\O$. For example,
$\O(U,v)$ denotes the smallest edge of $\cal E$ from $U$ to
$v$ whose packet has been opened.

The third part of the  data structure is for blossoms.
A blossom with $s$ nodes has {\it rank} $\f{\log s}$.
%Assume that in each operation $merge(A, B)$, $B$ is the larger blossom.
A {\it minimal blossom of rank $r$} is a blossom of rank $r$ resulting
from the {\it merge} of two blossoms of rank less than $r$.
Clearly the minimal blossoms of a given rank $r$ are
pairwise vertex disjoint.
Any blossom $B$ of rank $r$ contains a unique minimal blossom
$B_0$ of rank $r$.
The {\it minimal root} of $B$ is the root of $B_0$ in $T$.
It exists because of Lemma \ref{2.1lemma}.

The data structure for a blossom $B$ is as follows.
There are several bookkeeping items:
The rank $r$ and minimal root $b$ are recorded.
There is also a representation of the partition of $\cal O$ into blossoms.
A data structure for set merging \cite{T83} can be used: The 
blossom merging operation
$merge(A,B)$ executes a set merging operation  $union(A,B)$
to construct the new blossom; for any vertex $v$,
the set merging operation $find(v)$
gives the blossom currently containing $v$.

For simplicity the algorithms of Sections 2.2 -- 2.3
omit the obvious details associated with this bookkeeping.
We can also ignore the
time and space. For suppose we use
a simple set merging algorithm
that does one $find$ in $O(1)$ time, all $unions$ in $O(n\log n)$
time, and uses $O(n)$ space (e.g., \cite{AHU}). Clearly 
the space and the time for $unions$ are within the desired bounds for Edmonds'
algorithm; the time for $finds$ can be associated with  other
operations. Hence we shall ignore this bookkeeping.

The heart of the blossom data structure is
a Fibonacci heap ${\cal F}(B)$ for each blossom $B$.
Every vertex of $B$ has all its packets of rank at most $r$ opened.
Heap ${\cal F}(B)$ has two types of entries:

\b

\i Each of the first $3 \d 2^r$ ancestors $v$ of $b$ 
(the minimal root of $B$) has an entry.
The heap key of $v$ is $\O(B,v)$ if $v\notin B$; it is $\infty$ if
$v\in B$.
%an edge $xv$ with smallest cost possible subject
%to the constraint that $x\in B$ and 
%$xv$ is in a packet of $x$ that has been opened.

\ii Each unopened packet $P$ of a vertex of $B$
has an entry. The key of $P$ is $smallest(P)$.

\b

\noindent
The entry for $B$ in heap ${\cal F}_0$ is the minimum of ${\cal F}(B)$.

A given vertex $v$ may simultaneously have entries
in a large number of heaps 
${\cal F}(B)$. (This occurs when $v$ is an ancestor of a large
number of vertices minimal roots $b$.) 
The algorithm must be able to find the entry for a given $v$
in a given ${\cal F} (B)$ in $O(1)$ time. To do this,
each blossom $B$ of rank $r$ has an array
$vertex_B[1\ ..\ 3\d 2^r]$ of pointers to the vertex entries in 
${\cal F} (B)$ -- specifically $vertex_B[i]$ gives the entry for the
ancestor of $b$ at depth $d(b)-i$. Thus given an ancestor $v$ the 
corresponding entry in 
${\cal F}(B)$ is $vertex_B[d(b)-d(v)]$.

The correctness of 
the data structure amounts to the following result, which shows that
${\cal F}_0$ contains the correct information for each blossom.

\begin{lemma}
\label{2.2lemma} At any time for any blossom $B$,
the minimum entry in ${\cal F}(B)$ equals $smallest(B,O-B)$.
\end{lemma} 

\begin{proof}
 Let $B$ have rank $r$.
%
% More precisely this amounts to two properties:
% Let $v$ be a vertex in a blossom $B$ of rank $r$, with
% an edge $vw$ in a packet $P$.
% If $P$ has been opened, then $w$ has an entry in ${\cal F}(B)$.
% If $P$ is unopened, then any blossom containing both
% $B$ and $w$ has rank greater than $r$.
First observe that a blossom containing both ends of an edge of rank $r$ 
has rank at least $r$. This follows from Lemma 2.1.
It justifies the fact that the data structure for $B$ 
does not open any packet $P$ of rank more than $r$:
%Any edge in $P$ certainly goes to a vertex not in $B$.
if
a blossom step is done for $smallest(P)$, this will
increase the rank of the blossom so that a new blossom data structure
gets initialized (in the new data structure $P$ gets opened).

Next observe that
if a packet containing an edge $vw$, $d(v)>d(w)$, has been opened
then $w$ has an entry in ${\cal F}(B)$.
This follows from two inequalities:
Since the packet is opened its rank is at most $r$, whence
$d(w)> d(v)-2^{r+1}$. Since the rank of $B$ is $r$, 
less than $2^r$ vertices have been to its minimal rank $r$
blossom. Thus $d(v)>d(b)-2^r$.
Transitivity implies $d(w)>d(b)- 3\d 2^r$, i.e., $w$ has an entry in
${\cal F}(B)$.
Clearly it suffices that the entry for $w$ maintains $\O(B,w)$ --
an edge in an opened packet
that leads to $w$ but is not $\O(B,w)$ is irrelevant.

These two observations show that
${\cal F}(B)$ contains all possible candidates for $smallest(B,O-B)$.
Furthermore each finite entry in ${\cal F}(B)$ corresponds to an edge from $B$
to $O-B$. Thus the data structure is correct. 
\end{proof}

The four blossom merging operations are implemented so that they maintain the
defining properties of the data structure. A $make\_blossom$ operation
simply updates the representation of the partition of $\cal O$ into
blossoms. As already noted a $find\_min$ operation is trivial
given the heap ${\cal F}_0$. Now we describe the two
other operations.

Consider $make\_edge(vw,t)$, where $d(v)>d(w)$ and $v$ is in blossom
$B$. Compute the rank of $vw$ as $r=\f{\log (d(v)-d(w)) }$.
If $r$ is at most the rank of $B$ then $vw$ belongs to an opened
packet. Update the key for $w$ in ${\cal F}(B)$ by possibly doing a
Fibonacci heap {\it decrease\_key} operation
(find the heap entry for $w$ using $vertex_B[d(b)-d(w)]$).
Otherwise use $packet_v[r]$ to find the unopened packet $P$.
Add $vw$ to $P$, updating $smallest(P)$ and the
corresponding Fibonacci heap entry if necessary. 
Finally if the minimum of ${\cal F}(B)$ decreases do a {\it
decrease\_key} operation for $B$'s entry in ${\cal F}_0$.

Consider {\it merge}$(A,B)$. Let $C$ denote the blossom resulting from the
merge. Suppose first that $C$ has the same rank $r$ as one of its
constituents, say $B$; clearly $A$ has rank less than $r$.
The algorithm forms the data structure for $C$
by reading the information for $A$ into the data structure for $B$.
More precisely the following is done. The data structure for $B$ is now
associated with $C$, e.g., ${\cal F}(B)$ is now ${\cal F}(C)$.
Entries for vertices in ${\cal F}(A)$ are used to update entries for
vertices in ${\cal F}(C)$ by possibly doing {\it decrease\_key}
operations.
Packets of $A$ with rank at most $r$ are opened
and their edges are used to update entries for vertices in ${\cal F}(C)$.
Each unopened packet of $A$ is inserted into ${\cal F}(C)$.
The Fibonacci heap operation $delete\_min$ is done in
${\cal F}(C)$ as long as the minimum entry is a vertex in $C$.
The entries for $A$ and $B$ in ${\cal F}_0$ are deleted and replaced by
the new heap minimum in ${\cal F}(C)$.

The second case for $merge(A,B)$ is
when $C$ has a larger rank $r$ than either constituent.
(Thus $C$ is a minimal blossom of rank $r$.) 
The algorithm begins by initializing a new data structure for $C$.
The information for both $A$ and $B$ is read into this data
structure, following the procedure of the first case.

Correctness of these algorithms is obvious -- they 
maintain the invariants of the data structure.
We show the entire blossom merging algorithm
achieves the desired resource bounds,
$O(m+n\log^2 n)$ time and $O(m+n\log n)$ space.
To do this we make a preliminary observation: Over the entire algorithm,
the total number of vertex entries in all distinct heaps ${\cal F}(B)$ 
is $O(n\log n)$. To show this note that the distinct heaps correspond to
the heaps of minimal blossoms $B$ of each rank $r$. Such a blossom $B$ 
contains at least $2^r$ vertices and ${\cal F}(B)$ has $O(2^r)$ vertex
entries. As already noted 
the minimal blossoms of rank $r$ are pairwise vertex disjoint.
Thus the distinct heaps for rank $r$ have $O(n)$ vertex entries.
This implies the desired total of $O(n\log n)$ vertex entries.

Now we show the space bound. The  $packet_v$ tables use  $O(n\log n)$
space. 
The heaps ${\cal F}(B)$ use $O(n\log n)$ space, since 
at any given time there are $O(n)$ heap entries for vertices and 
$O(n\log n)$ entries for packets. (For vertices, note that 
at any time the existing blossoms are pairwise vertex disjoint.)
In addition the $vertex_B$ tables are stored.
At any time the existing heaps ${\cal F}(B)$
have a total of $O(n)$ entries in these tables. This
does not necessarily imply a space
bound of $O(n)$, since contiguous space must be allocated dynamically as 
blossoms grow. Instead of introducing a space allocation strategy we
simply note that the total size of all tables ever existing is $O(n\log
n)$, by the preliminary observation.
It is clear that the remaining space is $O(m)$,
so the desired space bound follows.

Next we prove the time bound. An
operation $make\_blossom(A)$ uses $O(|A|)$ time.
A $find\_min$ operation uses $O(1)$ time and a
$make\_edge$ operation uses $O(1)$ amortized time. This amounts to
$O(m)$ time total. It remains only to estimate the time for all {\it merge}
operations.

As observed above there are $O(n\log n)$ 
vertex entries in all distinct Fibonacci heaps.
Each such entry can be deleted, using $O(n\log^2n)$ time total.
Similarly each
vertex entry can cause a {\it decrease\_key} when it is transferred
to a larger heap, using $O(n\log n)$ time total.
Each packet gets inserted in $O(\log n)$ distinct heaps ${\cal F}(B)$,
using $O(n\log^2n)$ time total. It gets deleted from a heap only once,
right before that heap is discarded, using $O(n\log n)$ time.
Each edge uses $O(1)$ time when its packet is opened.
These contributions dominate the total time.
We conclude that the simple merging algorithm works as desired.

\subsection {The refined merging algorithm}
\label{RefinedAlgSec}
This section implements Edmonds' algorithm with the desired efficiency,
$O(m+n\log n)$ time and $O(m)$ space. 
It does this by presenting an algorithm for tree-blossom merging
that uses the same resources.
(We still assume the tree operations  of Section 3.)

We start by describing a useful operation, also used in \cite{GGS}. 
Consider a blossom $B$ and a set $A$ of
consecutive ancestors of $B$. Let $S$ be a set of edges from opened
packets, each joining $A$
and $B$, containing the edge $\O(B,a)$ for each $a\in A$.
To {\it clean $S$} means to discard all edges of $S$ except the edges
$\O(B,a)$, $a\in A$.

A cleaning operation can be done in time $O(|A|)$ plus
$O(1)$ per edge discarded, and space $O(|A|)$.
To do this suppose $A$ consists of the ancestors of $B$ with depths
in the range $[\ell..h]$. Read the edges of $S$ into
an array $A[\ell..h]$, where
$A[i]$ keeps track of the smallest edge from $B$ to the depth
$i$ ancestor.

Now we describe the data structure for the refined algorithm. 
It is based on this classification: A blossom is
{\it small} if it has less than $\f{\log n}$ vertices. Otherwise it is
{\it big}.

Consider a small blossom $B$. Let $S$
denote the set of edges of $\cal E$ that are incident to $B$.
The edges of $S$ are stored in two data
structures associated with $B$, a packet ${\cal P}(B)$ and a 
list ${\cal L}(B)$. ${\cal P}(B)$ uses 
the data structure of Section 2.2 for packets (i.e., a linked list), but
in addition to having a pointer to the first
element ${\cal P}(B)$ has a pointer to the last element. 
${\cal P}(B)$ contains all edges of $S$ that have rank at least
$\f{\log n}$.
It is natural to think of ${\cal L}(B)$ as containing edges of a
fictitious packet that has been opened.  Thus the function
$\O$ takes into account all edges ever in ${\cal L}(B)$. 
${\cal L}(B)$ contains edges of $S$ with
rank less than $\f{\log n}$
joining $B$ to $O-B$;
for each vertex $a$ adjacent to $B$ along such an edge,
${\cal L}(B)$ contains $\O(B,a)$ and possibly other edges incident to $a$. 
The entry for $B$ in ${\cal F}_0$ is 
$smallest( {\cal P}(B) \cup {\cal L}(B) )$. 

This data structure is correct --
the entry for $B$ in ${\cal F}_0$ is 
the same as the desired entry $smallest( B, O-B)$. 
To show this observe that  ${\cal P}(B) \cup {\cal L}(B)$ contains  
$smallest( B, O-B)$ by the above discussion. 
Furthermore ${\cal P}(B) \cup {\cal L}(B)$ contains  
only edges leading out of $B$. This follows because an edge of ${\cal P}(B)$ 
has rank larger than $B$. 

Observe also that ${\cal L}(B)$ contains edges leading to $O(\log n)$
distinct ancestors of $B$.

Now we give the data structure for big blossoms.
It uses packets and heaps. We discuss these in turn.

For packets, consider a minimal big blossom $B$, i.e.,
$B$ has at least $\f{\log n}$ vertices but neither of its constituents does.
$B$ has $\f{\log n}+1$ packets, just like a vertex in the
simple algorithm. As in the simple algorithm
the packet of rank $r$ contains edges of rank $r$. (A difference is
that now edges in a packet of rank $r$ can lead to
vertices differing in depth by more than $2^{r+1}$.)
The packets for $B$ are maintained throughout the algorithm, even when
$B$ gets absorbed into larger blossoms $C$.
(In fact after $B$ gets absorbed, edges may get added to its packets.
These edges will be incident to $C$ but need not be incident to $B$.)
Note that there are $O(n)$ such packets total, since
there are $O(n/\log n)$ such blossoms $B$, each with $O(\log n)$
packets.

For heaps, consider a big blossom $B$ with rank $r$
(thus $r\ge \l2 n$). Let $b$ be its minimal root.
$B$ has a Fibonacci heap ${\cal F}(B)$, that is the same as in the
simple algorithm (see \i -- \ii of the discussion of heaps in Section
2.2) with one change, in how the ancestors  of $b$ are 
processed. The first $3\cdot2^{r}$ ancestors of $b$
are partitioned into {\it groups} of $\f{\log n}$ consecutive vertices.
Groups are treated like vertices in the simple algorithm.
Specifically, ${\cal F}(B)$ has one entry for each group $G$. The
key for $G$ is  $\O(B,G-B)$. (This is infinite if $G\con B$.)
Each group $G$ has a list ${\cal L}(G)$ of edges of $\cal E$ from $B$ to $G$;
${\cal L}(G)$ contains $\O(B,w)$ for each vertex $w\in G$, if it
exists, and possibly other edges incident to $w$.
Finally there is an array $group_B[1\ ..\ 
\c   { \frac{ 3\cdot 2^r}{ \f{\log n} }} ]$ HAL IS THIS RIGHT 
of pointers to the groups ($group_B[i]$ points to the group of
ancestors of $b$ with depths in the range $(d(b)-(i-1)\f{\log n} \ ..\ 
d(b)-i\f{\log n}]$\ ).
Note that over the entire algorithm there are $O(n)$ groups total. This
follows since the minimal blossoms for rank $r$ collectively contain at
most $n$ vertices. Since these blossoms are all big they collectively 
contain $O(n/\log n)$ groups.

The algorithm maintains the invariant that the packets for all blossoms
included in a big blossom $B$ collectively contain all edges incident to
$B$. (Thus when a vertex enters a big blossom for the first time
its edges are placed in packets of the appropriate rank.
This is true even if the packet has been opened, by convention.)
The entry for a big blossom $B$ in
heap ${\cal F}_0$ is the minimum entry in ${\cal F}(B)$. The same
reasoning as in the
simple algorithm shows this entry is correct.

Now we sketch the algorithms using these data structures.
We also show that each algorithm achieves the desired time bound,
and uses permissible auxiliary space.
The operations $make\_blossom$ and $find\_min$ are straightforward,
as in the simple algorithm.

Consider $make\_edge(vw,t)$, where  $d(v)>d(w)$ and
$v$ is in blossom $B$. The rank $r$ of $vw$ is computed.
If $B$ is small then 
$vw$ is added to ${\cal P}(B)$ or ${\cal L}(B)$, depending on the rank
$r$. 
The entry for $B$ in ${\cal F}_0$ is updated if appropriate.
Suppose $B$ is big.
If $r$ is greater than the rank of $B$ then $vw$ belongs in an unopened
packet; an unopened packet of rank $r$ for some blossom in $B$
is chosen arbitrarily and $vw$ is added to it.
Otherwise (when $r$ is at most the rank of $B$)
the group $G$ for $w$ is found (using
$group_B[ \c {   \frac{d(b)-d(w)} {\f{\log n}}   } ]$) and $vw$ is 
added to 
${\cal L}(G)$. In both cases,
{\it decrease\_key} is done in the heaps ${\cal F}(B)$
and ${\cal F}_0$ if appropriate.

It is clear that $make\_edge$ uses $O(1)$ (amortized) time.
This depends on the fact that lists ${\cal L}(B)$ and ${\cal L}(G)$
do not get cleaned when an edge is added.

Next consider an operation $merge(A,B)$. 
\fi

